How the Analyzer can Help the User Help the Analyzer

The automation offered by modern program proof tools goes hand in hand with the capability to interact with the tool when the verification fails. The SPARK proof tool tries to help the user by providing the right information, so that the user can help the tool complete the proof. In this article, we present these mechanisms and how they work concretely on a simple running example.

==> eptcsdata.tex <==
\providecommand{\firstpage}{97}
\providecommand{\publicationstatus}{A. Paskevich, J. Proen\c{c}a (Eds.): Formal Integrated\\
Development Environment 2021 (F-IDE 2021)\\
EPTCS 338, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.338.12}{10.4204/EPTCS.338.12}}
\pdfoutput=1

